Improved Matrix Gaussian Mechanism for Differential Privacy

The wide deployment of machine learning in recent years gives rise to a great demand for large-scale and high-dimensional data, for which the privacy raises serious concern. Differential privacy (DP) mechanisms are conventionally developed for scalar values, not for structural data like matrices. Our work proposes Improved Matrix Gaussian Mechanism (IMGM) for matrix-valued DP, based on the necessary and sufficient condition of $ (\varepsilon,\delta) $-differential privacy. IMGM only imposes constraints on the singular values of the covariance matrices of the noise, which leaves room for design. Among the legitimate noise distributions for matrix-valued DP, we find the optimal one turns out to be i.i.d. Gaussian noise, and the DP constraint becomes a noise lower bound on each element. We further derive a tight composition method for IMGM. Apart from the theoretical analysis, experiments on a variety of models and datasets also verify that IMGM yields much higher utility than the state-of-the-art mechanisms at the same privacy guarantee.

==> algorithm.tex <==
\section{Privacy and Utility}\label{Sec_alg}
We show in this section that IMGM has form to be optimized w.r.t. the utility subspace. If we know some dimensions/directions of the matrix are more important than others, we can select noise distributions such that less noise is inserted to the more important part of the matrix, at the cost of a higher level of noise adding to the less important part. By treating the IMGM theorem as a differentially-private constraint, we formulate the problem from an optimization perspective. A closed-form solution is obtained which minimizes the total impact of the noise on the output, and the form of the solution is scalable to large-size problems. Based on the solutions, the algorithms are proposed with numeral calculations. 

Assume the task has linear utility subspace such that: 
\begin{equation*}
{Y} = W_1 f({X}) W_2^{\top},
\end{equation*}
where $f({X}) \in \mathbb{R}^{m \times n}$, $ {W_1} \in \mathbb{R}^{m^{\prime} \times m},~{W_2} \in \mathbb{R}^{ n^{\prime} \times n} $ represents the utility subspace. % $ \mathbf{b} \in \mathbb{R}^{J_1 \times J_{2} \times \cdots \times J_{N}} $ is a constant bias. 
$ {Y} \in \mathbb{R}^{m^{\prime} \times n^{\prime}} $ is the output. 
%The model are mostly found in linear regression/classification and fully-connected neural networks. 这个确实不敢保证
To preserve privacy, we apply IMGM by sampling a noise $\mathcal{Z} \sim \mathcal{MN}_{m,n}(\mathbf{0},\Sigma_{1},\Sigma_2)$ and make predictions on the perturbed query result:
\begin{equation*}
\hat{{Y} }={W_1}  [f({X}) + \mathcal{Z}] W_2^{\top}.
\end{equation*}

According to \cite{li2015matrix,geng2015optimal} and other mechanisms, we define our objective as the error on the original query result, measured by the expected norm of weighted noise. If the error is minimized, it means less perturbation is done to the output. The goal is to minimize:
\begin{equation}
\underset{{U}_1 , U_2}{\min}  ~\mathbb{E}\|{Y} - \hat{{Y} } \|_F^{2} 
\Leftrightarrow ~ \underset{U_1, U_2}{\min} ~\mathbb{E}\| W_1 U_1 N U_2^{\top} W_2^{\top} \|_F^{2},
\end{equation}
by Def. \ref{lemma:TVG}, we could get $ \mathcal{Z} = U_1 N U_2^{\top} $. And $ N $ is a matrix valued Gaussian variable with every element follows $ \mathcal{N}(0,1) $. Then calculate the expection of the equation above:
\begin{equation}
\mathbb{E}\| W_1 U_1 N U_2^{\top} W_2^{\top} \|_F^{2} = \| W_1 U_1\|_F^2 \| W_2 U_2\|_F^2.
\end{equation}
The detailed calculation process will be presented in the appendix. 
Therefore, the goal is to:
\begin{equation}
\underset{U_1, U_2}{\min} ~\| W_1 U_1\|_F^2 \| W_2 U_2\|_F^2.
\end{equation}
%由于DP的限制条件只针对协方差矩阵的奇异值，而对于其方向矩阵 没有限制，因此在设计矩阵噪声是存在很大的空间。这里我们在确定协方差矩阵的奇异值的情况下，给出其方向矩阵的最优的策略（使误差最小）。
Since the limitation of Differential Privacy is only for the singular value of the covariance matrices, and there is no restriction on its directional matrix, there is a lot of space for the design of matrix noise. Here we give the optimal strategy for its direction matrix (to minimize the error) with the fixed  singular value of the covariance matrices.
\begin{equation}
\min_{W_{U_1}}\| W_1 U_1\|_F^2 = \sum_{i=1}^{m}  \sigma_i^2(W_1) \sigma_{m-i+1}^2(U_1)
\end{equation}

Therefore, we can get the optimization problem with the optimal directional matrices. By using the optimal directional matrices together with the differential private constraint from Thm.~\ref{thm: IMGM}, we can rewrite the constraint and formulate the problem as the following optimization problem:
\begin{equation}\label{IMGM_opt}
\begin{split}
\underset{U_1, U_2}{\min} ~&\left(\sum_{i=1}^{m} \sigma_{i}^2(W_1){\sigma}_{m-i+1}^2(U_1)\right)\left(\sum_{i=1}^{n} \sigma_{i}^2(W_2){\sigma}_{n-i+1}^2(U_2)\right), ~~\\
\text{s.t.} & ~~ \sigma_{m-i+1}(U_1) \sigma_{n-i+1}(U_2) \geq \frac{s_2(f)}{B},~i \in [r] ,\\
& ~~\sigma_1(U_1) \geq \cdots \geq \sigma_m(U_1) \geq 0,\\
& ~~\sigma_1(U_2) \geq \cdots \geq \sigma_n(U_2) \geq 0.
\end{split}
\end{equation}

The full proof are given in the Supplementary materials. We give the closed from of the optimization problem:
\begin{equation}
\begin{split}
\sigma_{1}(U_1) = \cdots= \sigma_{m}(U_1), ~~\sigma_{1}(U_2) = \cdots= \sigma_{n}(U_2) \\
\sigma_{i}(U_1) \sigma_{j}(U_2) = \frac{s_2(f)}{B}, ~~\forall ~ 1\le i \le m, 1 \le j \le n,
\end{split}
\end{equation}
And the minimun value is 
\begin{equation}
\frac{s_2^2(f)}{B^2}\left(\sum_{i=1}^{m} \sigma_{i}^2(W_1)\right)\left(\sum_{i=1}^{n} \sigma_{i}^2(W_2)\right)
\end{equation}


\begin{algorithm}
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{Caculate Privacy Bound}
	\label{alg: privacy bound}
	\begin{algorithmic}[1] 
		\REQUIRE (a) privacy parameters $\epsilon,\delta$.
		\ENSURE privacy bound $ \hat{B} $ and the variance $ \sigma $
		\STATE {Let $\delta_{0}=\Phi(0)-e^{\varepsilon} \Phi(-\sqrt{2 \varepsilon})$}
		\IF {$\delta \geq \delta_{0}$} 	 
		\STATE { Define $B_{\varepsilon}^{+}(v)=\Phi(\sqrt{\varepsilon v})-e^{\varepsilon} \Phi(-\sqrt{\varepsilon(v+2)})$ }
		\STATE {Compute $v^{*}=\sup \left\{v \in \mathbb{R}_{\geq 0}: B_{\varepsilon}^{+}(v) \leq \delta\right\}$}
		\STATE {Let $\alpha=\sqrt{1+v^{*} / 2}-\sqrt{v^{*} / 2}$}
		\ELSE	
		\STATE { Define $B_{\varepsilon}^{-}(u)=\Phi(-\sqrt{\varepsilon u/T})-e^{\varepsilon} \Phi(-\sqrt{\varepsilon(u+2)})$ }
		\STATE {Compute $u^{*}=\inf \left\{u \in \mathbb{R}_{\geq 0}: B_{\varepsilon}^{-}(u) \leq \delta\right\}$}
		\STATE {Let $\alpha=\sqrt{1+u^{*} / 2}+\sqrt{u^{*} / 2}$}
		\ENDIF
		\STATE {Let $ \hat{B} = \sqrt{2\varepsilon}/\alpha $}
		\STATE {Let $ \sigma = s_2^2(f)/\hat{B }$}
		\RETURN {$\hat{B}$ and $ \sigma $}
	\end{algorithmic} 
\end{algorithm}

%\begin{algorithm}
%	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%	\renewcommand{\algorithmicensure}{\textbf{Output:}}
%	\caption{Caculate Privacy Bound}
%	\label{alg: privacy bound}
%	\begin{algorithmic}[1] 
%		\REQUIRE (a) privacy parameters $\epsilon,\delta$, (b) number of epochs T
%		\ENSURE privacy bound $ \hat{B} $ and the 
%		\STATE {Let $\delta_{0}=\Phi(0)-e^{\varepsilon} \Phi(-\sqrt{2 \varepsilon/T})$}
%		\IF {$\delta \geq \delta_{0}$} 	 
%		\STATE { Define $B_{\varepsilon}^{+}(v)=\Phi(\sqrt{\varepsilon v/T})-e^{\varepsilon} \Phi(-\sqrt{\varepsilon(v+2)/T})$ }
%		\STATE {Compute $v^{*}=\sup \left\{v \in \mathbb{R}_{\geq 0}: B_{\varepsilon}^{+}(v) \leq \delta\right\}$}
%		\STATE {Let $\alpha=\sqrt{1+v^{*} / 2}-\sqrt{v^{*} / 2}$}
%		\ELSE	
%		\STATE { Define $B_{\varepsilon}^{-}(u)=\Phi(-\sqrt{\varepsilon u/T})-e^{\varepsilon} \Phi(-\sqrt{\varepsilon(u+2)/T})$ }
%		\STATE {Compute $u^{*}=\inf \left\{u \in \mathbb{R}_{\geq 0}: B_{\varepsilon}^{-}(u) \leq \delta\right\}$}
%		\STATE {Let $\alpha=\sqrt{1+u^{*} / 2}+\sqrt{u^{*} / 2}$}
%		\ENDIF
%		\STATE {Let $ B = \sqrt{2\varepsilon/T}/\alpha $}
%		\STATE {Let $ \sigma = s_2^2(f)/B $}
%		\RETURN {$B$ and $ \sigma $}
%	\end{algorithmic} 
%\end{algorithm}





